Impact Evaluation of Falsified Data Attacks on Connected Vehicle Based Traffic Signal Control

Connected vehicle (CV) technology enables data exchange between vehicles and transportation infrastructure and therefore has great potentials to improve current traffic signal control systems. However, this connectivity might also bring cyber security concerns. As the first step in investigating the cyber security of CV-based traffic signal control (CV-TSC) systems, potential cyber threats need to be identified and corresponding impact needs to be evaluated. In this paper, we aim to evaluate the impact of cyber attacks on CV-TSC systems by considering a realistic attack scenario in which the control logic of a CV-TSC system is unavailable to attackers. Our threat model presumes that an attacker may learn the control logic using a surrogate model. Based on the surrogate model, the attacker may launch falsified data attacks to influence signal control decisions. In the case study, we realistically evaluate the impact of falsified data attacks on an existing CV-TSC system (i.e., I-SIG).

==> comments_ieee.tex <==
WAI COMMENTS:

My major comment is that we have to be very careful about the use of words to avoid giving an impression that we are teaching how people can attack the system. The followings are some of my key comments:
1) Avoid using "we SHOW HOW attackers can ...", which sounds like we are teaching people how to attack the system and the paper is a show-how. We only FOUND that that kind of attack is possible and we wanna evaluate its impact with an ultimate good heart of protecting our system
2) Avoid using wordings, like "attackers can ... attackers can ... attackers then ...", which sounds like a step-by-step manual.
3) Avoid using wordings, like "an attack policy is proposed".  We DID NOT PROPOSE any attack policy. The so-called simple attack policy is only our ASSUMED attack policy that we think similar policies could potentially be adopted by attackers.
4) We did not adopt/propose a surrogate model that could be an example for attackers to learn the control logic and how to attack. We only use the decision tree regression/classification to MODEL a representative surrogate model that we think similar models could potentially be leveraged by attackers.



IEEE COMMENTS:

The paper needs some improvements:
1) The survey should include some of the work done on attacks and security of RSUs and traffic signals. Several well-known papers are missing.
2) The main contribution of the paper is very weak, only small section of the paper. More work need to be done.
3) Increase size of Fig 5.


===================================

Comments:
you missed many references to support your claims starting from the 1st page some abbreviations were not described making the paper hard to follow sometimes the related work section should not include the threat model or the (2) attacks you mentioned.

your white box black box definition is correct for software testing but not for security evaluation.
 assuming that the attacked knows the code makes the defender's job much harder. so if you managed to prove that your system is secure even if the source code is available that actually makes you a more attractive solution to buy.

assuming that attackers will not have access to the code as mentioned in the intro is wrong, even if the code was not open-sourced,  reverse engineering can be very helpfull revealing the logic behind the binaries.

finally, you mentioned that you tested your system with a naive attack, is that a good way to show that your system is good or even acceptable given the mission-critical nature of the application.
finally
general presentation and results figures, legends needs your review


===================================
The paper makes practically no technical contribution at all. The authors seem to be unaware of related work. Also the technical contribution is also very weak.

The authors should really rethink the entire paper. The first thing they need do is a thorough literature search. With this done, they need to redefine the problem they're trying to solve.






==> edit_log.tex <==

May 12, 2020
revise threat model
change false data injection attack to falsified data attack
change (false data/trajectory) to (falsified data/trajectory) 


May 6, 2020
1) revise the ring-barrier figure
2) move Attack Model to Threat Model, revise the problem that the attacker tries to solve (maximize dissimilarity)
3) in the defense part, remove I-SIG-50\%; briefly discuss two directions of defense strategies
4) other minor changes


